On Runtime Enforcement via Suppressions

Runtime enforcement is a dynamic analysis technique that uses monitors to enforce the behaviour specified by some correctness property on an executing system. The enforceability of a logic captures the extent to which the properties expressible via the logic can be enforced at runtime. We study the enforceability of Hennessy-Milner Logic with Recursion (muHML) with respect to suppression enforcement. We develop an operational framework for enforcement which we then use to formalise when a monitor enforces a muHML property. We also show that the safety syntactic fragment of the logic, sHML, is enforceable by providing an automated synthesis function that generates correct suppression monitors from sHML formulas.

==> sections/lts.tex <==
\noindent
\textbf{\textsf{Labelled Transition Systems:}}
Labelled Transition Systems (LTSs) provide a convenient framework for defining an operational description of the behaviour of a system. An LTS, is a triple $\langle\Proc,\Act,\rightarrow\rangle$ which is composed from:
\begin{enumerate}[$(i)$]
	\item a set of \emph{states}, $\pV,\pVV,\pVVV\in\Proc$, corresponding to processes;
	\item a set of \emph{actions}, $\actu,\actg\in\Act$, which include all the system's \emph{observable} ($\acta,\actb\in\CEvt$) and \emph{internal} $\actt\notin\Evt$ actions; and
	%\item a set of \emph{actions}, $\actu,\actg\in\Act=\CEvt\cup\set{\actt}$, which include all the system's \emph{observable} concrete events $\acta,\actb\in\CEvt$, along with a distinguished silent action $\actt\notin\Evt$, denoting \emph{unobservable} internal system operations; and 
	\item a \emph{transition} relation, $\reduc\;\subseteq(\Proc\times\Act\times\Proc)$ that relates the state on the RHS, to the other state on the LHS of the transition via a unidirectional reduction from left to right over a specific action, \eg $(\pV,\acta,\pV')\in\reduc$ describes a unidirectional reduction from state \pV to $\pV'$ over action \acta.
\end{enumerate} 

\begin{figure}[t]
	\textbf{Syntax}
	\begin{align*}
	\pV,\pVV,\pVVV\in\Proc & \bnfdef \nil && (\text{inaction}) &&
	 \bnfsepp \prf{\actu}{\pV} && (\text{prefixing}) &&
%	 \bnfsepp \ch{\pV}{q} && (\text{choice})\\
	 \bnfsepp \chBigI\,\pV_i && (\text{choice}) \\ 
	& \bnfsepp \rec{x}{\pV} && (\text{recursion}) && 
	 \bnfsepp x && (\text{rec. variable})
	\end{align*}
	\textbf{Dynamics}
	\begin{mathpar}
		\inference[\rtit{Act}]{}{\prf{\actu}{\pV}  \traSS{\actu} \pV} 
		\and
%		\inference[\rtit{SelL}]{\pV \traSS{\actu} \pV'}{\ch{\pV}{\pVV}  \traSS{\actu} \pV'}  
%		\and  
%		\inference[\rtit{SelR}]{\pVV \traSS{\actu} \pVV'}{\ch{\pV}{\pVV}  \traSS{\actu} \pVV'} 
%		\and
		\inference[\rtit{Sel}]{\pV_j \traSS{\actu} \pVV_j}{\chBigI\,\pV_i \traSS{\actu} \pVV_j}[$j\in\IndSet$] 
		\and
		\inference[\rtit{Rec}]{\pV\sub{\rec{\rV}{\pV}}{\rV} \traSS{\actu} \pV'}{\rec{\rV}{\pV} \traSS{\actu} \pV'}  
	\end{mathpar}	
	\caption{A Model for describing Systems}
	\label{fig:lang}
\end{figure}

For convenience, we define processes, \Proc, using the \emph{regular fragment} of CCS \cite{Milner1992CCS} as defined by the syntax in \Cref{fig:lang}.   Assuming a specific set of (visible) concrete events, $\acta$ and a denumerable set of (recursion) variables $\rV,\rVV,\rVVV\in\Vars$, processes are defined as either the \emph{inactive process} \nil, an \emph{action-prefixed process} \prf{\actu}{\pV} \ie prefixed by an action $\actu$ where \actu is either a visible (\acta) or a silent (\actt) action, a \emph{mutually-exclusive choice} amongst processes where $\chBigI\,\pV_i$ sums up the processes identified by the unique indices in \IndSet (such that $\chBigI\,\pV_i$ represents $\ch{\pV_1}{\ch{\ldots}{\pV_n}}$, where $1,\ldots,n\in\IndSet$), or a \emph{recursive process} where \rec{x}{\pV} acts as a \emph{binder} for $\rV$ in $\pV$. We work up to alpha-conversion of bound recursion variables and assume that all recursive processes are guarded, meaning that all occurrences of bound recursion variables occur under an action prefix (either directly or indirectly). Closed terms are processes where all occurrences of recursion variables are bound.

% Occasionally, inactive processes are omitted when describing systems such that $\pV$ is written instead of $\nil \paral \pV$ or $\pV \paral \nil$ and $\prf{\acta}{\prf{\actb}{\nil}}$ as $\prf{\acta}{\actb}$; in order to lighten the presentation of our example derivations, we also implicitly work up to associativity and commutativity of parallel compositions where, for example, $\pV\paral q$ is some times treated as $q \paral \pV$. \footnote{These are normally expressed as structural equivalence rules such as $\pV\paral \nil \equiv \pV$ and $\pV\paral q \equiv q\paral \pV$ in standard CCS.  We elide them here to alleviate our exposition.}

When describing the dynamic behaviour of processes, we use the more intuitive notation $\pV\traS{\actu}\pV'$ in lieu of $(\pV,\actu,\pV')\in\reduc$, along with notation $\pV\ntraS{\actu}$ to denote $\lnot(\exists\pV'\cdot\pV\traS{\actu}\pV')$. The rules in \Cref{fig:lang} are standard. Rule \rtit{Act} allows a \actu-prefixed process $\prf{\actu}{\pV}$ to reduce over action \actu to the derivative \pV, \ie $\prf{\actu}{\pV}\traS{\actu}\pV$, while by rule \rtit{Sel}, a choice process, $\chBigI\,\pV_i$ reduces to $\pVV_j$ whenever there exists a process identified by some index $j\in\IndSet$ in this summation, \ie $\pV_j$ which performs a \actu-transition, \ie $\pV_j\traS{\actu}\pVV_j$ (\resp $\pVV\traS{\actu}\pVV'$). By rule \rtit{Rec}, a recursive process $\rec{\rV}{\pV}$ can reduce to $\pV'$ over action \actu, \ie $\rec{\rV}{\pV} \traSS{\actu} \pV'$, when its unfolded version, $\pV\sub{\rec{\rV}{\pV}}{\rV}$, reduces to $\pV'$ over \actu, \ie $\pV\sub{\rec{\rV}{\pV}}{\rV} \traSS{\actu} \pV'$.

We also employ the usual notation $\pV \wreduc \pV'$ and $\pV \wtraS{\acta} \pV'$ to denote weak transitions representing $\pV (\traS{\actt})^{\ast} \pV'$ and $\pV \wreduc\cdot\traS{\acta}\cdot\wreduc \pV'$ \resp, referring to $\pV'$ as a \actu-derivative of $\pV$. We also employ notation $\pV\wtraS{\hat{\actu}}\pV'$ to collectively refer to $\pV \wreduc \pV'$ and $\pV \wtraS{\acta} \pV'$. Sequences of visible actions are expressed as traces $\tr,\trr \in \CEvt^\ast$, such that sequences of transitions are defined as $\pV\wtra{\acta_1}\ldots\wtra{\acta_n} p_n$ as $\pV \wtraS{\tr} p_n$, where a trace $\tr = \acta_1,\ldots,\acta_n$. For more details, consult standard texts such as \cite{Milner1992CCS,Aceto2007Book}.

\begin{figure}[t]
	\begin{center}
		\begin{tikzpicture}[>=latex,auto,thick, scale=0.9]
			\begin{scope}[draw=blue!50,fill=blue!20,minimum size=0.5cm]
				\node (p1) at ( 0,0) [shape=circle,draw,fill] {$\pV_1$};
				\node (p2) at (-3,0) [shape=circle,draw,fill] {$\pV_2$};
				\node (p3) at ( 3,0) [shape=circle,draw,fill] {$\pV_3$};
				\node (p4) at ( 4.5,0)  {\phantom{$\pV_4$}};
				\end{scope}
				\begin{scope}[draw=blue!50,fill=blue!50]
				\draw[->] (p1) [bend left=30] to node {\footnotesize\actReq} (p2); 
				\draw[->] (p2) [bend left=30] to node {\footnotesize\actAns} (p1); 
				\draw[->] (p1) to node[below] {\footnotesize\actCls} (p3);
			\end{scope}
		\end{tikzpicture}	
		\begin{tikzpicture}[>=latex,auto,thick, scale=0.9]
			\begin{scope}[draw=blue!50,fill=blue!20,minimum size=0.5cm]
			\node (q1) at ( 0,0) [shape=circle,draw,fill] {$\pVV_1$};
			\node (q2) at (-3,0) [shape=circle,draw,fill] {$\pVV_2$};
			\node (q3) at ( 3,0) [shape=circle,draw,fill] {$\pVV_3$};
			%\node (q4) at ( 4.5,0)  {\phantom{$\pVV_4$}};
			\end{scope}
			\begin{scope}[draw=blue!50,fill=blue!50]
			\draw[->] (q1) [in=30,out=80,loop] to node {\footnotesize\actReq} (q1); 
			\draw[->] (q1) [bend left=30] to node {\footnotesize\actReq} (q2); 
			\draw[->] (q2) [bend left=30] to node {\footnotesize\actAns} (q1); 
			\draw[->] (q1) to node[below] {\footnotesize\actCls} (q3);
			\end{scope}
		\end{tikzpicture}
		\begin{tikzpicture}[>=latex,auto,thick, scale=0.75]
			\begin{scope}[draw=blue!50,fill=blue!20,minimum size=0.5cm]
			\node (r1) at ( 0,2) [shape=circle,draw,fill] {$\pVVV_1$};
			\node (r2) at ( 4,2) [shape=circle,draw,fill] {$\pVVV_2$};
			\node (r3) at ( 4,-2) [shape=circle,draw,fill] {$\pVVV_3$};
			\node (r4) at ( 0,-2) [shape=circle,draw,fill] {$\pVVV_4$};
			\node (r5) at ( 2,0) [shape=circle,draw,fill] {$\pVVV_5$};
			\node (r6) at ( 7,3)  {\phantom{$\pVV_7$}};
			\end{scope}
			\begin{scope}[draw=blue!50,fill=blue!50]
			\draw[->] (r1) to node {\footnotesize\actReq} (r2); 
			\draw[->] (r2) to node {\footnotesize\actAns} (r3); 
			\draw[->] (r3) to node {\footnotesize\actCls} (r5);
			
			\draw[->] (r3) to node {\footnotesize\actReq} (r4); 
			\draw[->] (r4) to node {\footnotesize\actAns} (r1); 
			\draw[->] (r1) to node {\footnotesize\actCls} (r5);
			\end{scope}
		\end{tikzpicture}
		\begin{tikzpicture}[>=latex,auto,thick, scale=0.9]
		\begin{scope}[draw=blue!50,fill=blue!20,minimum size=0.5cm]
		\node (n0) at ( 0,0) [shape=circle,draw,fill] {$\pVVVV_1$};
		\node (n1) at ( 0,-2) [shape=circle,draw,fill] {$\pVVVV_2$};
		\node (n2) at (-3,0) [shape=circle,draw,fill] {$\pVVVV_3$};
		\node (n3) at ( 3,0) [shape=circle,draw,fill] {$\pVVVV_4$};
		\node (n4) at ( 0,-3)  {\phantom{$\pVVVV_3$}};
		\end{scope}
		\begin{scope}[draw=blue!50,fill=blue!50]
		\draw[->] (n0)  to node [right] {\actt} (n1); 
		\draw[->] (n1)  to node {\footnotesize\actReq} (n2); 
		\draw[->] (n2)  to node {\footnotesize\actAns} (n0); 
		\draw[->] (n1) to node[below] {\footnotesize\actCls} (n3);
		\end{scope}
		\end{tikzpicture}	
	\end{center}	
	\caption{A depiction of the system in \Cref{ex:lts}}
	\label{fig:ex:lts}
\end{figure}

%\begin{remark}
%	To alleviate the complexity of our examples, we omit the process id when describing input and output operations, \ie we specify $\actAns$ instead of $\send{i}{v}$ and $\recv{}{v}$ instead of $\send{i}{v}$ (for any process id $i$). \qed
%\end{remark}

\begin{example}
	\label{ex:lts}
	Consider a (reactive) system that acts as a server that is identified with process id $i$, and which repeatedly accepts \emph{requests} and subsequently responds by outputting an \emph{answer}, with the possibility of terminating through the special \emph{close} request (\actN{cls}). Such a system may be expressed as the following process, $\pV_1$.
	\begin{displaymath}
		\pV_1=\procPVdef
	\end{displaymath}
	We can outright notice that process $\pV_1$ is designed to output an answer (\actAns) for every input request (\actReq). The \emph{same} behaviour can also be represented by processes $\pVVV_1$ and $\pVVVV_1$ (below), which differ from $\pV_1$ since $\pVVV_1$ is an \emph{unfolded} version of $\pVVV_1$, while $\pVVVV_1$ performs an internal \actt action before inputting a request.
	\begin{align*}
		\pVVV_1\defeq&\;\rec{\rV}{\bigl(\ch{\prf{\actReq}{ \prf{\actAns}{\bigl(\underline{\ch{\prf{\actReq}{\prf{\actAns}{\rV}}}
						{\prf{\actCls}{\nil}}}\bigr) }}}{\prf{\actCls}{\nil}}\bigr)} \\
		\pVVVV_1\defeq&\;\rec{\rV}{\bigl(\ch{\prf{\underline{\,\actt\,}}{ \prf{\actReq}{ \prf{\actAns}\rV}}}{\prf{\actCls}{\nil}}\bigr)}
	\end{align*}
	By contrast, process $\pVV_1$ denotes a server that, although similar to $\pV_1$, can also \emph{non-deterministically} refuse to answer for a given request.
	\begin{displaymath}
		\pVV_1=\pVVAdef
	\end{displaymath}
	Pictorially, the \resp LTSs denoted by processes $\pV_1$, $\pVV_1$, $\pVVV_1$ and $\pVVVV_1$ may be represented by the graphs in \Cref{fig:ex:lts}, where the nodes correspond to processes and the arcs correspond to transitions, $\traS{\actu}$.   \qed
\end{example}

%\paragraph{Bisimilarity of LTSs}
%Intuitively, a \emph{bisimulation} \cite{Aceto2007Book,Milner1992CCS} is a binary relation that associates the behaviour of two Labelled Transition Systems that \emph{exhibit the same behaviour}, \ie in a way that one system \emph{simulates} the other and vice versa. Variants of bisimulation includes \emph{Strong and Weak Bisimulation} (see \Cref{def:strong-bisim,def:weak-bisim}, below). 
%
%\begin{definition}[Strong Bisimulation]\label{def:strong-bisim}
%	\renewcommand{\qedsymbol}{ \;}
%	A binary relation \R is a \emph{Strong Bisimulation relation} whenever $(\pV,\pVV)\in\R$, such that
%	\begin{enumerate}[(a)]
%		\item if $\pV\traS{\actu}\pV'$ then there exists a \emph{strong transition} $\pVV\traS{\actu}\pVV'$ such that $(\pV',\pVV')\in\R$  \qed
%		\item if $\pVV\traS{\actu}\pVV'$ then there exists a \emph{strong transition} $\pV\traS{\actu}\pV'$ such that $(\pV',\pVV')\in\R$ \qed
%	\end{enumerate}
%\end{definition}
%
%Hence, for a pair of processes, $(\pV,\pVV)$, to be in a \emph{Strong Bisimulation relation}, it is required that each process is able to simulate both visible (\acta) and internal (\actt) actions of the other process, \eg if $\pV\traS{\acta}\pV'$ then $\pVV\traS{\acta}\pVV'$ and if $\pVV\traS{\actt}\pVV'$ then $\pV\traS{\actt}\pV'$. By contrast, \emph{Weak Bisimulation} abstracts away from internal (\actt) actions, \ie each process is only required to simulate the visible actions of the other process, and can thus simulate visible actions after performing a zero or more internal (\actt) transitions, \eg if $\pV\traS{\acta}\pV'$ then $\pVV\traS{\actt}^{\ast}\traS{\acta}\traS{\actt}^{\ast}\pVV'\,\equiv\,\pVV\wtraS{\acta}\pVV'$ and if $\pVV\traS{\actt}\pVV'$ then $\pV\traS{\actt}^{\!0}\!\!\pV'$.
%
%\begin{definition}[Weak Bisimulation]\label{def:weak-bisim}
%	\renewcommand{\qedsymbol}{ \;}
%	A binary relation \R is a \emph{bisimulation relation} whenever $(\pV,\pVV)\in\R$, such that
%	\begin{enumerate}[(a)]
%		\item if $\pV\traS{\actu}\pV'$ then there exists a \emph{weak transition} $\pVV\wtraS{\hat{\actu}}\pVV'$ such that $(\pV',\pVV')\in\R$ \qed
%		\item if $\pVV\traS{\actu}\pVV'$ then there exists a \emph{weak transition} $\pV\wtraS{\hat{\actu}}\pV'$ such that $(\pV',\pVV')\in\R$ \qed
%	\end{enumerate} 
%\end{definition}
%
%
%\paragraph{Proving Bisimilarity of LTS processes} 
%Since \emph{Strong (}\resp\emph{Weak) Bisimilarity} is the \emph{largest} Strong (\resp Weak) Bisimulation relation, proving that two LTS processes \pV and \pVV are Strong (\resp Weak) Bisimilar, \ie $\pV\bisim\pVV$ (\resp $\pV\wbisim\pVV$), only requires showing that there exists a Strong (\resp Weak) bisimulation relation \R that can relate them as stated by \Cref{def:strong-bisim,def:weak-bisim}. Note that since Strong Bisimilarity is \emph{stricter} than its Weak counterpart, two Strong bisimilar processes are inherently Weak bisimilar as well.
%
%However, proving the contrary \ie $\pV{\not\bisim}\pVV$ (\resp $\pV{\not\wbisim}\pVV$) is not as straight forward. In fact, to show that a process \pV is \emph{not} Strong (\resp Weak) bisimilar to \pVV, we must show that \emph{every} binary relation that exists between \pV and \pVV \emph{do not satisfy} \Cref{def:strong-bisim} (\resp \Cref{def:weak-bisim}), and hence do not constitute towards valid bisimulation relations. Given the lack of practicality of this exhaustive approach, a \emph{game characterization for Strong (\resp Weak) bisimulation} \cite{Aceto2007Book,Stirling1996} is generally employed to prove that two LTS processes are either \emph{bisimilar} ($\pV\bisim\pVV$) or \emph{not} ($\pV{\not\bisim}\pVV$); in the former case, a relation \R can be deduced from the game derivation. The definition for a bisimulation game is given below. For more information regarding the bisimulation game characterisation one may consult Appendix \Cref{sec:app:bisim-games} or standard texts such as \cite{Aceto2007Book,Stirling1996}.
%
%\begin{example}[Proving Strong Bisimilarity]\label{ex:strong-bisim-p-r}
%	To prove that $\pV_1\bisim\pVVV_1$, consider the following relation \R,
%	\[\R\defeq\Set{(\pV_1,\pVVV_1),(\pV_2,\pVVV_2),(\pV_1,\pVVV_3), (\pV_2,\pVVV_4), (\pV_3,\pVVV_5)}\]
%	Since $\pV_1\bisim\pVVV_1$ is the largest strong bisimulation relation relating processes $\pV_1$ and $\pVVV_1$, it thus suffices showing that relation \R is a Strong Bisimulation Relation as stated by \Cref{def:strong-bisim}; we prove that this is true as follows:
%	\begin{proofn}[$\;\;\pmb{\pV_1\bisim\pVVV_1}$]
%		To prove that the pair $(\pV_1,\pVVV_1)\in\R$ satisfies \Cref{def:strong-bisim}, we show that $\pV_1\traS{\actReq}\pV_2$ can be \emph{strongly simulated} by $\pVVV_1\traS{\actReq}\pVVV_2$ and vice-versa, such that the resultant process pair $(\pV_2,\pVVV_2)\in\R$ is \emph{true}. In addition, we show that similarly reduction $\pV_1\traS{\actCls}\pV_3$ can be simulated by $\pVVV_1\traS{\actCls}\pVVV_5$ and vice-versa, such that $(\pV_3,\pVVV_5)\in\R$ is also \emph{true}.
%		
%		The same argument applies for pairs $(\pV_2,\pVVV_2)$, $(\pV_1,\pVVV_3)$ and $(\pV_2,\pVVV_4)$, \ie
%		\[
%		\begin{array}{rl}
%			(\pV_2,\pVVV_2): & \pV_2\traS{\actAns}\pV_1 \emph{ bisimulates } \pVVV_2\traS{\actAns}\pVVV_3 \text{ such that } (\pV_1,\pVVV_3)\in\R \text{ is \emph{true}.}\\
%			(\pV_1,\pVVV_3): & \pV_1\traS{\actReq}\pV_2 \emph{ bisimulates } \pVVV_3\traS{\actReq}\pVVV_4 \text{ such that } (\pV_2,\pVVV_4)\in\R \text{ is \emph{true}.}\\
%			\hfill \text{ and} & \pV_1\traS{\actCls}\pV_3 \emph{ bisimulates } \pVVV_3\traS{\actAns}\pVVV_5 \text{ such that } (\pV_3,\pVVV_5)\in\R \text{ is \emph{true}.}\\			 
%			(\pV_2,\pVVV_4): & \pV_2\traS{\actAns}\pV_1 \emph{ bisimulates } \pVVV_4\traS{\actAns}\pVVV_1 \text{ such that } (\pV_1,\pVVV_1)\in\R \text{ is \emph{true}.}
%		\end{array}
%		\]
%		
%		\noindent Finally, since both processes in the pair $(\pV_3,\pVVV_5)$ are unable to perform any further reductions, \ie $\pV_3\ntraS{\actu}$ and $\pVVV_5\ntraS{\actu}$, they still satisfy the constraints of \Cref{def:strong-bisim}.
%		
%	\end{proofn}$\\$
%	\noindent Hence, with the above proof we can conclude that relation \R is a \emph{Strong Bisimulation relation}, such that since $(\pV_1,\pVVV_1)\in\R$, we can also conclude that $\pV_1\bisim\pVVV_1$.
%	 
%	Similarly, to prove that $\pV_1\bisim\pVVVV_1$, we must once again find a binary relation and prove that it is a Strong Bisimulation Relation as defined by \Cref{def:strong-bisim}. Hence, we consider relation $\R'$,
% 	\[\R'\defeq\Set{(\pV_1,\pVVVV_1),(\pV_1,\pVVVV_2),(\pV_2,\pVVVV_3), (\pV_3,\pVVVV_4)}\]
% 	From the case of $(\pV_1,\pVVVV_1)\in\R'$, we can immediately notice that relation $\R'$ is \emph{not} a Strong Bisimulation relation since reduction $\pV_1\traS{\actReq}\pV_2$ cannot be strongly simulated by process $\pVVVV_1$, \ie $\pVVVV_1\ntraS{\actReq}$. Hence, from relation $\R'$ we are \emph{unable to conclude} whether $\pV_1\bisim\pVVVV_1$ or not. 
% 	
% 	However, as proven below, by abstracting over internal (\actt) transitions, by \Cref{def:weak-bisim} we can conclude that relation $\R'$ is a \emph{Weak Bisimulation} relation.
% 	\begin{proofn}[$\;\;\pmb{\pV_1\wbisim\pVVVV_1}$]
% 		To prove that the pair $(\pV_1,\pVVVV_1)\in\R'$ satisfies \Cref{def:weak-bisim}, we show that transitions $\pV_1\traS{\actReq}\pV_2$ and $\pV_1\traS{\actCls}\pV_3$ can be \emph{weakly simulated} as $\pVVVV_1\traS{\actt}\traS{\actReq}\pVVVV_3$ and $\pVVVV_1\traS{\actt}\traS{\actCls}\pVVVV_4$ \resp, such that $(\pV_2,\pVVVV_3)\in\R'$ and $(\pV_3,\pVVVV_4)\in\R'$ are both true; while transition $\pVVVV_1\traS{\actt}\pVVVV_2$ can also be weakly simulated as $\pV_1\traS{\actt}^{0}\pV_1$, where $(\pV_1,\pVVVV_2)\in\R'$ is \emph{true}.
% 	 	
% 	 	In the case of $(\pV_1,\pVVVV_2)\in\R'$, we show that transitions $\pV_1\traS{\actReq}\pV_2$ and $\pV_1\traS{\actCls}\pV_3$ can be simulated by $\pVVVV_2\traS{\actReq}\pVVVV_3$ and \resp by $\pVVVV_2\traS{\actCls}\pVVVV_4$, such that $(\pV_2,\pVVVV_3)\in\R'$ is true and $(\pV_3,\pVVVV_4)\in\R'$ is true as well; dually, $\pVVVV_2\traS{\actReq}\pV_3$ and $\pVVVV_2\traS{\actCls}\pVVVV_4$ can also be simulated by $\pV_1\traS{\actReq}\pV_2$ and \resp by $\pV_1\traS{\actCls}\pV_3$. 
% 	 	
% 	 	Finally, we know that the pair $(\pV_3,\pVVVV_4)\R'$ satisfies the constraints of \Cref{def:weak-bisim} since neither of the two processes can perform a \actu-reduction.
% 	 	
% 	\end{proofn}$\\$
%	\noindent Since $\R'$ is a Weak Bisimulation relating processes $\pV_1$ and $\pVVVV_1$, we can therefore conclude that $\pV_1\wbisim\pVVVV_1$. \qed
%\end{example}
%
%One may already notice that processes $\pV_1$ and $\pVV_1$ from \Cref{fig:ex:lts} appear to behave differently even when observed as a black box from an external perspective; this is because $\pV_1$ is \emph{always} obliged to provide an answer to an external request, while $\pVV_1$ may occasionally refuse to do so. 
%
%In general, proving that $\pV_1{\not\bisim}\pVV_1$ is an exhaustive technique that requires proving that \emph{all binary relations} \R that can relate processes $\pV_1$ and $\pV_2$ are \emph{not} a Strong Bisimulation; this inherently proves that there \emph{does not exist} some Strong Bisimulation relation \R, such that $(\pV_1,\pVV_1)\in\R$. Alternatively, the bisimulation game characterisation provides a more practical alternative to formally prove that $\pV_1\not\bisim\pV_2$ (see Appendix \Cref{sec:app:bisim-games} for more details).
%

